Distributed Decisions on Optimal Load Balancing in Loss Networks

When multiple users share a common link in direct transmission, packet loss and network collision may occur due to the simultaneous arrival of traffics at the source node. To tackle this problem, users may resort to an indirect path: the packet flows are first relayed through a sidelink to another source node, then transmitted to the destination. This behavior brings the problems of packet routing or load balancing: (1) how to maximize the total traffic in a collaborative way; (2) how self-interested users choose routing strategies to minimize their individual packet loss independently. In this work, we propose a generalized mathematical framework to tackle the packet and load balancing issue in loss networks. In centralized scenarios with a planner, we provide a polynomial-time algorithm to compute the system optimum point where the total traffic rate is maximized. Conversely, in decentralized settings with autonomous users making distributed decisions, the system converges to an equilibrium where no user can reduce their loss probability through unilateral deviation. We thereby provide a full characterization of Nash equilibrium and examine the efficiency loss stemming from selfish behaviors, both theoretically and empirically. In general, the performance degradation caused by selfish behaviors is not catastrophic; however, this gap is not monotonic and can have extreme values in certain specific scenarios.

==> intro.tex <==

%--------------------------------------------
\section{Introduction}

Since the seminal work of Erlang \cite{erlang1917solution}, loss networks have been widely studied as mathematical models for various stochastic systems where different types of resources are used to serve diverse classes of customers involving simultaneous resource possession and nonbacklogging workloads. Various applications include  database systems \cite{mitra1984probabilistic}, wireless networks \cite{momvcilovic2011linear}, and telecommunication systems \cite{mitra1996atm} (see an overview in \cite{jung2019revisiting}). E.g., in packet-switching telecommunication networks, packet losses may occur either due to buffer overflows (these are congestion losses) or random non-congestion losses that are due to the transmission channel (e.g., a radio channel).



Many works study the routing games or load balancing games in loss networks \cite{altman2014routing,bean1997braess,toure2020congestion}, where selfish users want to balance their workloads  on the nodes or lossy links  to minimize the amount of packet losses. For example, in distributed computer systems jobs or transactions continuously arrive and  need to be processed by computers; in communication networks packets are transmitted through communication links, and transportation flow networks have incoming threads of vehicles to drive through roads, etc. The well-studied problem is, how can a centralized planner schedule the workloads to maximize the system efficiency, and how the dynamic in a decentralized environment develops. 


%\czrev{
%Many works study the routing games or load balancing games in loss networks \cite{altman2014routing,bean1997braess,toure2020congestion}, where selfish users \czcom{try to minimize their own packet losses with link selection.}
%% 郑策：selfish is selft-interested, but selft-interested is not selfish
%\czdel{For example, in distributed computer systems jobs or transactions continuously arrive and  need to be processed by computers,} In communication networks, packets may be lost due to collisions, i.e., over two packets arrive during the same transmission period. To mitigate this problem, users may choose to relay their packets to another source via sidelink

%are either directly transmitted to the base station or indirectly via relays.


%\czdel{and transportation flow networks have incoming threads of vehicles to drive through roads, etc.} The well-studied problem is, how can a centralized planner schedule the workloads to maximize the system efficiency, and how the dynamic in a decentralized environment develops. 

%}

%In this paper, we consider the load balancing in a communication loss network consisting of $m$ source nodes  (e.g., servers, host computers or processors) $\{s_1,\ldots,s_m\}$ and one destination node $d$. Each source $s_i$ has $n_i$ users seeking for service, and the traffic of packets originating from each user is assumed to follow an independent Poisson point process with identical rate $\phi$. The nodes in the network are connected by two types of communication links: side  links that connect two sources, and direct links that connect a source to the destination. The side  links have random non-congestion losses, and the direct links have congestion losses that depend on the arrival rate and service rate of each server.


In this paper, we consider the load balancing in a communication loss network consisting of $m$ source nodes  (e.g., servers, host computers or processors) $\{s_1,\ldots,s_m\}$ and one destination node $d$. Each source $s_i$ has $n_i$ users seeking service, and packets flow from each user follows an independent Poisson arrival process with identical rate $\phi$.
The nodes in the network are connected in two types of links: side links between two sources, and direct links between a source to the destination. The side links have random non-congestion losses, and the direct links have congestion losses that depend on the arrival rate and service rate of each server. The user cannot split its trafﬁc, and has to decide how to route all its  traffic from the source node  to the destination node. 
There are two {transmission strategies}: a direct path (DP) in which the packet goes directly from the source to the destination, and a two-hop indirect path (IP) in which the packet is first relayed (forwarded) to another source node and then takes the direct link from that node to the destination.


%While the users in classic routing games usually have additive costs (such as delays or tolls) \cite{patriksson2015traffic}, in the loss networks considered,  the costs of users are the  packet loss probability,  which is non-additive and even non-convex. Each user wants to minimize the loss probability, and the users may play a game by strategically choosing their own path (DP or IP). We say a state is \textit{Nash equilibrium} (NE) of the game, if no user can decrease its loss probability by unilateral deviation.  The concept of NE is of special importance from a dynamic standpoint \cite{orda1993competitive}: in a practical scenario, a user changes its route dynamically and repeatedly, in response to the varying load conditions, and the stability points in such systems are exactly those in which no user can gain by changing. 


Unlike the additive costs (such as delay or fees) in classical routing games \cite{patriksson2015traffic},  this paper views the  packet loss probability for each user as the performance metric, which is non-additive and even non-convex.
Each user attempts to minimize its loss probability and engage in a game by strategically choosing their own paths (DP or IP).
We say that a state is \textit{Nash equilibrium} (NE), if no user can reduce its loss probability by unilateral deviation. The concept of NE is of special importance for a dynamic standpoint \cite{orda1993competitive}: in a practical scenario, a user will dynamically and continuously change its route based on changing load conditions. In such a system, the stable points are precisely where no user can gain by deviating.
%The most related works are \cite{altman2014routing,toure2020congestion}. Both works consider a specific loss network with two source nodes, and each source have an equal number of users. Moreover, they only focus on a quite restricted case, in which the strategies of all users must be the same. We {study a more general setting} %generalize their setting 
%by considering multiple sources and different number of users, and abandoning the restrictions on users' strategies.  

%\czrev{
Building on \cite{altman2014routing,toure2020congestion} where a specific loss network of two source nodes with equal number of users is studied, we extend it to a general setting with multiple sources and different user numbers. What is more, the restriction that all users have same strategies is abandoned.
%}

% \subsection{Our contributions and organization}

%This work contributes to the load balancing game in three aspects: optimizing the system efficiency, characterizing Nash equilibrium, and measuring the efficiency loss of Nash equilibrium, both theoretically and empirically. Precisely, when a centralized planner exists {(who determines the paths of users)}, we propose an optimal algorithm that maximizes the total traffic rate of packets that are successfully transmitted. {When the users play a game} in a decentralized environment where distributed decisions are made by the autonomous and self-interested users, %continuously, it often converges to an equilibrium in which no user can decrease her loss probability by unilateral deviation. 
%we give sufficient and necessary conditions on Nash equilibrium, which depend on the number of users selecting DP and IP in each source, and which IP is selected.
%Further, since a Nash equilibrium may be suboptimal for the system efficiency, we use the {standard} notion \textit{price of anarchy} (PoA) %\cite{koutsoupias1999worst} to measure how the system  efficiency degrades due to the strategic behaviours of these selfish agents, compared with the system optimum achieved by a centralized planner. In the end, all theoretical findings are confirmed by experiments.


%\czrev{
Our work contributes to the load balancing game in three aspects: optimizing the system efficiency, characterizing Nash equilibrium, and measuring the efficiency loss of Nash equilibrium, both theoretically and empirically. Specifically, when a centralized planner exists, we propose an optimal algorithm that maximizes the total traffic rate, i.e., packets that are successfully transmitted. In a decentralized environment where distributed decisions are made by autonomous and self-interested users,
we derive sufficient and necessary conditions on Nash equilibrium, which depend on the number of users {on DP and each IP}.
Further, since a NE may be suboptimal for the system efficiency, we use the  \textit{price of anarchy} (PoA) \cite{koutsoupias1999worst} to measure how the system efficiency degrades due to the strategic behaviours of these selfish users, in comparison with the system optimum achieved by a centralized planner. In the end, {new findings and analysis are shown in simulations}.

%}


%\violetcomment{The formal model and notations are presented in Section \ref{sec:model}. In Section~\ref{sec:opt}, we propose an algorithm to find an optimal solution. Section~\ref{sec:ne_poa} give a characterization of NEs. In Section~\ref{sec:sim}, we provide numerical experiments that confirm our findings.}


==> pure_twosource.tex <==

\section{Two sources}\label{sec:twopure}

 This section is devoted to the special case of two sources (i.e., $m=2$). Assume w.l.o.g. that $n_1\ge n_2$. For notational convenience, for each user $i\in N$, we represent her strategy as a single variable $p_i\in\{0,1\}$, which is the probability of selecting DP. Accordingly, there is a unique IP, and the probability of selecting IP is $1-p_i$. Let $\mathbf p=(p_1,\ldots,p_n)$ be the strategy profile of all users. 

%---------------------------------------------------------
\iffalse
 Then \eqref{equ:11} can be simplified as
\begin{align}
    TR=\frac{T_1\mu}{T_1+\mu}+\frac{T_2\mu}{T_2+\mu}
\end{align}
where 
\begin{align}
    T_1&=u_1\phi+(n_2-u_2)(1-q)\phi\notag\\
    T_2&=u_2\phi+(n_1-u_1)(1-q)\phi\notag
\end{align}
\fi


%In this section, we consider the setting with two sources and $n_1\neq n_2$. Assume w.l.o.g. that $n_1\ge n_2$. Let $\boldsymbol\alpha=(\alpha_1,\ldots,\alpha_n)$ be the strategy profile of users, where $\alpha_i\in[0,\phi]$ denotes the traffic rate over DP for user $i\in N$.

We can rewrite the functions defined in Section \ref{sec:model} in a simpler way. Given strategy profile $\mathbf p$, define  $u_1=\sum_{i\in N_1}p_{i}$ to be the number of users in $N_1$ who choose DP, and $u_2=\sum_{j\in N_2}p_{j}$ to be the number of users in $N_2$ who choose DP. {Denote by $p=1-q$ the probability that a packet is not lost over a relay link.}
First, the traffic rate over link $(s_1,d)$ is given by
$$T_1(\mathbf p)=\sum_{i\in N_1}p_i\phi+\sum_{j\in N_2}\phi(1-p_j)p=u_1\phi+(n_2-u_2)p\phi,$$
and similarly, the traffic rate over link $(s_2,d)$ is
$$T_2(\mathbf p)=\sum_{j\in N_2}p_j\phi+\sum_{i\in N_1}\phi(1-p_i)p=u_2\phi+(n_1-u_1)p\phi.$$
Next, the loss rate of user $i\in N_1$ is
\begin{equation}\label{eq:33}
    LR_i(\mathbf p)=p_i\phi\frac{T_1}{T_1+\mu}+(1-p_i)q\phi+p\phi(1-p_i)\frac{T_2}{T_2+\mu},
\end{equation}
and the loss rate of user $j\in N_2$ is
\begin{equation}\label{eq:44}
    LR_j(\mathbf p)=p_j\phi\frac{T_2}{T_2+\mu}+(1-p_j)q\phi+p\phi(1-p_j)\frac{T_1}{T_1+\mu}.
\end{equation}
Then the total traffic rate is given by
\begin{align}
TR(\mathbf p)=&~\sum_{i\in N_1}(\phi-LR_i)+\sum_{j\in N_2}(\phi-LR_j)= \frac{T_1\cdot \mu}{T_1+\mu}+\frac{T_2\cdot\mu}{T_2+\mu}.\label{eq:trp}
\end{align}


%----------------------------------------------------------------

%We study the asymmetric case with two sources and $n_1\neq n_2$, but pure strategy, i.e., $p_{ki}=1$ or $0$, where $p_{k,i}$ is the probability that user $k\in N_i$ routes any arriving packet through DP $(s_i,d)$.

\iffalse
The system efficiency is measured by the total traffic rate defined below, and we want to maximize it.
\begin{align}\label{equ:11}
    TR:&=\sum_{i\in N_1}(\phi-LR_i)+\sum_{j\in N_2}(\phi-LR_j)\notag\\
       &=\mu\phi\left[(1-q)n_1\frac{1}{\mu+T_2}+\sum_{i\in N_1}p_{i1}\left(\frac{1}{\mu+T_1}-\frac{1-q}{\mu+T_2}\right)\right]\notag\\
       &+\mu\phi\left[(1-q)n_2\frac{1}{\mu+T_1}+\sum_{j\in N_2}p_{j2}\left(\frac{1}{\mu+T_2}-\frac{1-q}{\mu+T_1}\right)\right].
\end{align}

\Q{We give details to proof \eqref{equ:11} as below,
\begin{align*}
    \sum_{i\in N_1}(\phi-LR_i)&=\sum_{i\in N_1}\left(\phi-\left(p_{i1}\phi\frac{T_1}{T_1+\mu}+(1-p_{i1})\phi q+(1-q)(1-p_{i1})\phi\frac{T_2}{T_2+\mu}\right)\right)\\
    &=\phi\sum_{i\in N_1}\left(1-\left(p_{i1}\frac{T_1}{T_1+\mu}+(1-p_{i1}) q+(1-q)(1-p_{i1})\frac{T_2}{T_2+\mu}\right) \right)\\
    &=\phi\left[(1-q)n_1\frac{\mu}{\mu+T_1}+\sum_{i\in N_1}p_{i1}\left(-\frac{T_1}{\mu+T_1}+q+(1-q)\frac{T_2}{\mu+T_2}\right)\right]\\
    &=\phi\left[(1-q)n_1\frac{\mu}{\mu+T_1}+\sum_{i\in n_1}p_{i1}\left(1-\frac{T_1}{\mu+T_1}-(1-q)+(1-q)\frac{T_2}{\mu+T_2}\right)\right]\\
    &=\mu\phi\left[(1-q)n_1\frac{1}{\mu+T_1}+\sum_{i\in N_1}p_{i1}\left(\frac{1}{\mu+T_1}-\frac{1-q}{\mu+T_2}\right)\right]\\
\end{align*}}
\fi

We investigate the system optimum, NEs, and the PoA in the following.

%---------------------------------------------------------------------
\subsection{Computing the optimal solution}

As a centralized planner, one wants to maximize the total traffic rate $TR$ arriving at the destination $d$. Noting that $TR$ can be written as a function of $u_1,u_2$, the maximization problem is formulated by $\max_{u_1,u_2}\frac{T_1\mu}{T_1+\mu}+\frac{T_2\mu}{T_2+\mu}$, subject to $0\leq u_1\leq n_1, 0\leq u_2\leq n_2$ and $u_1,u_2\in\mathbb Z$.

\iffalse
We consider the linear program (LP) consisting of (\ref{lp:1}), (\ref{lp:2}) and (\ref{lp:3}), removing the integer constraints. \bluecomment{The optimum of LP is an upper bound on the true optimum with integer constraints, and it is very close to the true optimum  when the number of users are large enough.}  The Lagrange function of LP is given by:
\begin{align}
    \mathcal{L}(u_1,u_2,\lambda)=-\frac{T_1\mu}{T_1+\mu}-\frac{T_2\mu}{T_2+\mu}-\lambda_1 u_1-\lambda_2 u_2+\lambda_3 (u_1-n_1)+\lambda_4(u_2-n_2),
\end{align}
where $\lambda_1$ and $\lambda_2$ are  Lagrange multipliers for the constraints of $u_1\ge 0,u_2\ge 0$; $\lambda_3$ and $\lambda_4$ are  Lagrange multipliers for the constraints of $u_1\leq n_1,u_2\leq n_2$, respectively. The first-order derivation of Lagrangian with respect of $m_i$ ($i=1,2$) is
\begin{align}
   \frac{\partial  \mathcal{L}}{\partial u_1}&=-\frac{\mu^2\phi}{(T_1+\mu)^2}+\frac{p\mu^2\phi}{(T_2+\mu)^2}-\lambda_1+\lambda_3, \notag\\
   \frac{\partial  \mathcal{L}}{\partial u_2}&=-\frac{\mu^2\phi}{(T_2+\mu)^2}+\frac{p\mu^2\phi}{(T_1+\mu)^2}-\lambda_2+\lambda_4.
\end{align}
The Karush-Kuhn-Tucker (KKT) conditions are
\begin{align*}
       -\frac{\mu^2\phi}{(T_1+\mu)^2}+\frac{p\mu^2\phi}{(T_2+\mu)^2}-\lambda_1+\lambda_3&=0 \\
       -\frac{\mu^2\phi}{(T_2+\mu)^2}+\frac{p\mu^2\phi}{(T_1+\mu)^2}-\lambda_2+\lambda_4&=0\\
       \lambda_i&\ge 0~\text{for}~i=1,2,3,4\\
        0\leq u_1&\leq n_1\\
        0\leq u_2&\leq n_2\\
        \lambda_1u_1&=0\\
        \lambda_3(u_1-n_1)&=0\\
        \lambda_2u_2&=0\\
        \lambda_4(u_2-n_2)&=0.
\end{align*}
Since $n_1\ge n_2$, in an optimal solution $(u_1^*,u_2^*)$, it must be $u_2^*=0$.  Solving KKT conditions, we can have the following conclusion.
\fi


We simply denote a solution by $(u_1,u_2)$. Given $q<1$, define $val:=\frac{n_2+n_1p+(1-\sqrt p)\mu/\phi}{\sqrt p+p}$.

\begin{theorem}\label{thm:aopt}
If $n_1\sqrt{p}> n_2+(1-\sqrt p)\mu/\phi$, then  either $(\lfloor val\rfloor,n_2)$ or $(\lceil val\rceil,n_2)$ is an optimal solution. Otherwise, $(u_1^*,u_2^*)=(n_1,n_2)$ is an optimal solution.
\end{theorem}
\noindent\emph{Proof sketch.}
We first note that in an optimal solution $(u_1^*,u_2^*)$, there is no pair $(i,j)$ of users from $(N_1,N_2)$ who both select IP, as otherwise they can deviate to DP to avoid the loss over delay link and thus improve the total traffic.  
Since $n_1\ge n_2$, it must be $u_2^*=n_2$. %It is easy to see that, in an optimal solution $(u_1^*,u_2^*)$ that maximizes the total traffic rate, all users in $N_2$ choose DP $(s_2,d)$, and no more than $\frac{n_1-n_2}{2}$ users in $N_1$ choose IP $(s_1,s_2,d)$. So it must be $u_2^*=n_2$. 
Then the total traffic rate $TR$ can be written as a function of single variable $u_1$:
\begin{align*}
    TR(u_1)&=2-\frac{\mu}{T_1+\mu}-\frac{\mu}{T_2+\mu}\\
    &=2-\frac{\mu}{u_1\phi+\mu}-\frac{\mu}{n_2\phi+(n_1-u_1)p\phi+\mu}
\end{align*}
By computing the derivative, $TR(u_1)$ increases in interval $[0,val]$. Moreover, if $val< n_1$,  $TR(u_1)$ decreases in interval $[val,n_1]$. Hence, the maximum is reached when $u_1=\min\{val,n_1\}$. Taking the integer constraint into account, if $val< n_1$ (i.e., $n_1\sqrt{p}> n_2+(1-\sqrt p)\mu/\phi$), the optimal solution $(u_1^*,u_2^*)$ is either $(\lfloor val\rfloor,n_2)$ or $(\lceil val\rceil,n_2)$. If $val\ge n_1$, the optimal solution is $(n_1,n_2)$. %\ma{pending for refine}
\qed

% \begin{remark} Consider the relaxation linear program (LP) consisting of (\ref{lp:1}), (\ref{lp:2}) and (\ref{lp:3}). By the above analysis in the proof of Theorem \ref{thm:aopt}, the optimal solution of LP is $(u_1^*,u_2^*)=(\min\{val,n_1\},n_2)$. 
% We can take the optimum of LP as an estimation for the true optimum with integer constraints. It is actually an upper bound on the optimal total traffic rate. 
% \end{remark}

%---------------------------------------------------
\subsection{Characterization of NEs}

We will present a characterization of NEs in this section. Given an arbitrary strategy profile $\mathbf p$, define $(V_1,V_2,V_3,V_4)$ as a partition of $N$, where $V_1=\{i\in N_1~|~p_i=1\}$,  $V_2=\{i\in N_1~|~p_i=0\}$, $V_3=\{j\in N_2~|~p_j=1\}$ and $V_4=\{j\in N_2~|~p_j=0\}$. Clearly, all users in $V_1$ and $V_3$ choose DP, and all users in $V_2$ and $V_4$ choose IP.  Supposing $\mathbf p$ is a NE, we discuss the deviation of users in $V_1,V_2,V_3,V_4$ respectively. 



\begin{theorem}\label{thm:cha}
Let $\mathbf p$ be an arbitrary strategy profile for the game with two sources. Let $u_1$ and $u_2$ be the number of users in $N_1$ and $N_2$ who choose DP under $\mathbf p$, respectively. We have
\begin{itemize}
    \item[{\rm [1]}] when (a) $u_1=n_1,u_2<n_2$, or (b) $u_1=0,u_2>0$, $\mathbf p$ cannot be a NE;
    \item[{\rm [2]}] when $u_1\in[0,n_1),u_2\in[0,n_2)$, $\mathbf p$ is NE if and only if $u_1\ge t_1(u_2)-1$ and $u_2\ge t_2(u_1)-1$;
    \item[{\rm [3]}] when $u_1\in(0,n_1),u_2=n_2$, $\mathbf p$ is NE if and only if $u_1\in[t_1(u_2)-1,t_1(u_2)]$;
    \item[{\rm [4]}] when $u_1=n_1,u_2=n_2$, $\mathbf p$ is NE if and only if $n_1p\le q\mu/\phi+n_2+p$. %$u_1\le t_1(u_2)$ and $u_2\le t_2(u_1)$.
\end{itemize}
\end{theorem}

Given $\mathbf p$, let $(V_1,V_2,V_3,V_4)$ be a partition of $N$ as defined above. We discuss the four cases, respectively, and give a sufficient and necessary condition. 
Since every situation of $u_1,u_2$ is included in the above four cases, we complete a characterization.

An intuitive explanation for Case 4 is, when  the loss probability $q$ of transmission over link $(s_1,s_2)$ is large enough, no user prefers IP, and the profile that all users select DP is a NE. In addition, when there is no transmission loss over link $(s_1,s_2)$, i.e., $q=0$, every user prefers a source with fewer users. So the profile that all users select DP is a NE only if the users are balanced on the two sources as evenly as possible, that is, $n_1\le n_2+1$. 



%\begin{corollary}\label{cor:NE}
%A strategy profile with $u_1=n_1,u_2=n_2$ (i.e., all users choose DP) is NE, if and only if $n_1p\le q\mu/\phi+n_2+p$.
%\end{corollary}

%Next, based on Theorem \ref{thm:cha}, we give some interesting conclusions. 
Note that the condition $n_1\sqrt{p}\le n_2+(1-\sqrt p)\mu/\phi$ in Theorem \ref{thm:aopt} implies the condition that $n_1p\le q\mu/\phi+n_2+p$ in Theorem \ref{thm:cha} (4), we have the following. 

\begin{corollary}\label{cor:NE2}
If a strategy profile with $u_1=n_1,u_2=n_2$ is optimal, then it is also a NE. %\bluecomment{In particular, when $val\ge n_1$, PoA=1.}
\end{corollary}

\iffalse
By Theorem \ref{thm:cha} (2), a profile with $u_1=u_2=0$ is NE if $0\ge \frac{q\mu}{\phi}+n_1-p-n_2p^2$ and $0\ge \frac{q\mu}{\phi}+n_2-p-n_1p^2$. Roughly, $n_1-n_2$ should be at most 1, and the success probability $p$ of transmission should be near 1. 
\begin{corollary}\label{cor:55}
A strategy profile with $u_1=0,u_2=0$ is a NE, if and only if (a) $n_1=n_2+1,p=1$, or (b) $n_1=n_2,n_1(1-p^2)\le p-\frac{q\mu}{\phi}$. %$n_2p^2+p\ge n_1$.
\end{corollary}
\fi

Note that $u_1\ge t_1(u_2)-1$ and $u_2\ge t_2(u_1)-1$ cannot hold simultaneously when $q>\frac{2}{n}$, and $u_1\ge t_1(n_2)-1$ cannot hold when $n_1p< q\mu/\phi+n_2+p$.
\begin{corollary}\label{cor:uni}
When $n_1p< q\mu/\phi+n_2+p$ and $q>\frac{2}{n}$, the unique NE is that all users choose DP, i.e., $u_1=n_1,u_2=n_2$.
\end{corollary}

\iffalse
\begin{corollary}\label{cor:NE6}
If a strategy profile $\mathbf p$ with $u_1\in(0,n_1)$ and $u_2<n_2$ is NE, then it must have $u_1+(n_2-u_2)=u_2+(n_1-u_1)$, that is, the load of the two links $(s_1,d)$ and $(s_2,d)$ is the same.
\end{corollary}
\begin{proof}
Suppose $\mathbf p$ is a NE.  By Theorem \ref{thm:cha}, we have $u_1\ge t_1-1,u_2\ge t_2-1$. It follows from $u_2\ge t_2-1$ that $2pu_2\ge q\mu/\phi+u_1(1+p^2)+n_2p-p-n_1p^2\ge 2pu_1+n_2p-n_1p$\redcomment{it's incorrect}, which implies $u_1+(n_2-u_2)\le u_2+(n_1-u_1)$. Similarly, it follows from $u_1\ge t_1-1$ that $u_2+(n_1-u_1)\le u_1+(n_2-u_2)$. Therefore, we have $u_1+(n_2-u_2)=u_2+(n_1-u_1)$.
\end{proof}

\begin{corollary}\label{cor:NE00}
When $val< n_1$, if $(u_1,u_2)$ is NE with $u_1\in(0,n_1)$ and $u_2<n_2$, then it must have $p\ge 1-\frac{2}{n_1+n_2}$.
\end{corollary}
\begin{proof}
By Corollary \ref{cor:NE6}, $(u_1,u_2)$ is a NE only if
\begin{align*}
  & 2pu_2\ge q\mu/\phi+(u_2+\frac{n_1-n_2}{2})(1+p^2)+n_2p-p-n_1p^2\\
 \Leftrightarrow~~ &   (2p-1-p^2)u_2\ge q\mu/\phi+\frac{n_1}{2}-\frac{n_2}{2}-\frac{n_1p^2}{2}-\frac{n_2p^2}{2}+n_2p-p\\
 \Rightarrow~~ & 0\ge n_1(1-p^2)+n_2(2p-1-p^2)-2p\\
  \Rightarrow~~ & \frac{2p}{1-p}\ge n_1(1+p)-n_2(1-p)\ge (n_1+n_2)p\\
    \Rightarrow ~~& 2\ge (1-p)(n_1+n_2)\\
      \Rightarrow ~~& p\ge 1-\frac{2}{n_1+n_2}.
\end{align*}
\end{proof}
\fi


We end this subsection by  proving the existence of NE.

\begin{theorem}
For any game instance with two sources, there exists a NE with $u_1>0$ and $u_2=n_2$.
\end{theorem}
\begin{proof}
By Theorem \ref{thm:cha} (4), if $n_1p\le q\mu/\phi+n_2+p$, then the strategy profile that all users choose DP (i.e., $u_1=n_1,u_2=n_2$) is a NE. Otherwise, $n_1p> q\mu/\phi+n_2+p$. Let $\tilde m$ be an integer in interval $[\frac{q\mu/\phi+n_2+n_1p-p}{2p},\frac{q\mu/\phi+n_2+n_1p+p}{2p}]=[t_1(n_2)-1,t_1(n_2)]$, which always admits at least one integer. Note that $n_1>\frac{q\mu/\phi+n_2+n_1p+p}{2p}\ge \tilde m>0$. By Theorem \ref{thm:cha} (3), a strategy profile with $u_1=\tilde m$ and $u_2=n_2$ is a NE. 
\end{proof}

%-------------------------------------------------------
\subsection{Price of Anarchy}
In this section we study the efficiency loss of Nash equilibria, which is measured by the price of anarchy. First, we note that there exists instances with $PoA>1$, because when $n_2\sqrt{p}+(\sqrt p-p)\mu/\phi<n_1p< q\mu/\phi+n_2+p$ and $q>\frac{2}{n}$, by Corollary \ref{cor:uni} there is a unique NE (i.e., $u_1=n_1,u_2=n_2$), however, which is not an optimal solution by Theorem \ref{thm:aopt}. Next, we upper bound the PoA for all game instances. Define $c=\min\{\frac{n_2}{n_1p},\frac{n_2-1}{n_2+1}\}$. 
The proof is deferred to Appendix.

\begin{theorem}\label{thm:poa}
For any instance with two sources, the price of anarchy is $PoA\le 1+\frac{\mu/\phi}{n_2-2+c\mu/\phi}$.
In particular, when $n_2$ has a higher-order of $\mu/\phi$ (i.e., $\mu/\phi=o(n_2)$), the PoA approaches to 1. 
\end{theorem}
\iffalse
\begin{proof}
Given any game instance, let $opt$ be  an optimal solution. By Eq. (\ref{eq:trp}), the optimal total traffic rate is upper bounded by
\begin{align*}
    TR(opt)&=\mu\left(\frac{T_1(opt)}{T_1(opt)+\mu}-\frac{T_2(opt)}{T_2(opt)+\mu}\right)\\
    %&=\mu\left(2-\frac{\mu/\phi}{val+\mu/\phi}-\frac{\mu/\phi}{n_2+(n_1-val)p+\mu/\phi}\right)\\
    %&\le \mu\left(2-\frac{\mu/\phi}{n_1+\mu/\phi}-\frac{\mu/\phi}{n_2+n_1p+\mu/\phi}\right)\\
    &\le \mu\left(\frac{n_1}{n_1+\mu/\phi}+\frac{n_2+n_1p}{n_2+n_1p+\mu/\phi}\right).
\end{align*}

Let $\mathbf p$ be an arbitrary NE. If $\mathbf p$ falls in Case 2 of Theorem \ref{thm:cha}, the traffic rate is bounded by 
\begin{align*}
    TR(\mathbf p)&=\mu\left(2-\frac{\mu/\phi}{u_1+(n_2-u_2)p+\mu/\phi}-\frac{\mu/\phi}{u_2+(n_1-u_1)p+\mu/\phi}\right)\\
   &\ge \mu\left(2-\frac{\mu/\phi}{\frac{n_1-1}{2}+\frac{n_2p}{2}+\mu/\phi}-\frac{\mu/\phi}{u_2+(n_1-u_1)p+\mu/\phi}\right)\\
    &\ge \mu\left(2-\frac{\mu/\phi}{\frac{n_1-1}{2}+\mu/\phi}-\frac{\mu/\phi}{\frac{n_2+n_1p-1}{2}+\mu/\phi}\right)\\
    &=\mu\left(\frac{n_1-1}{n_1-1+2\mu/\phi}+\frac{n_2+n_1p-1}{n_2+n_1p-1+2\mu/\phi}\right),
\end{align*}
where  the first inequality comes from $u_1\ge t_1(u_2)-1$, and the second inequality comes from $u_2\ge t_2(u_1)-1$. After calculation and relaxation, we have 
$$\frac{TR(opt)}{TR(\mathbf p)}\le 1+\frac{\mu/\phi}{n_2-2+\frac{n_2-1}{n_2+1}\mu/\phi}.$$


If $\mathbf p$ falls in Case 3, the traffic rate  is bounded by 
\begin{align*}
    TR(\mathbf p)&=\mu\left(2-\frac{\mu/\phi}{u_1+\mu/\phi}-\frac{\mu/\phi}{n_2+(n_1-u_1)p+\mu/\phi}\right)\\
   &\ge \mu\left(2-\frac{\mu/\phi}{\frac{n_1-1}{2}+\frac{n_2}{2p}+\mu/\phi}-\frac{\mu/\phi}{n_2+\mu/\phi}\right)\\
   &=\mu\left(\frac{n_1-1}{n_1-1+2\mu/\phi}+\frac{n_2}{n_2+\mu/\phi}\right),
    %&\ge \mu\left(2-\frac{\mu/\phi}{\frac{n_1-1}{2}+\mu/\phi}-\frac{\mu/\phi}{\frac{n_2+n_1p-1}{2}+\mu/(2\phi)}\right),
\end{align*}
where  the first inequality comes from $u_1\ge t_1(n_2)-1$, and the second inequality comes from $u_1\le t_1(u_2)$. After calculation and relaxation, we have 
$$\frac{TR(opt)}{TR(\mathbf p)}\le \max\{1+\frac{\mu/\phi}{n_2+\frac{n_2}{n_1p}\mu/\phi},1+\frac{\mu/\phi}{n_1-2+\frac{n_1-1}{n_1+1}\mu/\phi}\}.$$


If $\mathbf p$ falls in Case 4, the traffic rate is 
\begin{align*}
    TR(\mathbf p)&=\mu\left(\frac{n_1}{n_1+\mu/\phi}+\frac{n_2}{n_2+\mu/\phi}\right).
    %&\ge \mu\left(2-\frac{2\mu/\phi}{n_2+\mu/\phi}\right).
\end{align*}
By a similar calculation, we have 
$$\frac{TR(opt)}{TR(\mathbf p)}\le 1+\frac{\mu/\phi}{n_2+\frac{n_2}{n_1p}\mu/\phi}.$$

Combining the above three cases, it completes the proof
\end{proof}

\fi
